A Vanilla Multi-Task Framework for Dense Visual Prediction Solution to 1st VCL Challenge -- Multi-Task Robustness Track

In this report, we present our solution to the multi-task robustness track of the 1st Visual Continual Learning (VCL) Challenge at ICCV 2023 Workshop. We propose a vanilla framework named UniNet that seamlessly combines various visual perception algorithms into a multi-task model. Specifically, we choose DETR3D, Mask2Former, and BinsFormer for 3D object detection, instance segmentation, and depth estimation tasks, respectively. The final submission is a single model with InternImage-L backbone, and achieves a 49.6 overall score (29.5 Det mAP, 80.3 mTPS, 46.4 Seg mAP, and 7.93 silog) on SHIFT validation set. Besides, we provide some interesting observations in our experiments which may facilitate the development of multi-task learning in dense visual prediction.

==> sections/related_work.tex <==
\section{Related Work}

\subsection{LiDAR-based 3D Object Detection}

3D object detection aims to detect instances in the 3D space, which is of great importance in various applications, such as autonomous driving, navigation robot, and augmented reality. 
Current LiDAR detectors \cite{yin2021center,zhou2018voxelnet,yang20203dssd} mainly voxelize the point cloud into a BEV or voxel representations and adopt traditional 2D convolutions to predict bounding boxes. To improve the inference speed, some works \cite{fan2021rangedet,liang2020rangercnn} attempt to detect objects directly through the range view. \cite{zhou2020end} combines both BEV and range-view features together to achieve better performance. VoxelNet \cite{zhou2018voxelnet} adopts PointNet \cite{qi2017pointnet} to extract local features through raw point clouds and fill them into the predefined voxel space. PointPillar \cite{lang2019pointpillars} directly processes points inside a pillar to naturally formulate BEV feature representations, establishing an ultra-fast baseline detector. Inspired by CenterNet \cite{duan2019centernet}, CenterPoint \cite{yin2021center} introduces a center-based label assignment strategy in 3D object detection, achieving competitive detection accuracy among various approaches. In addition to dense one-stage detectors, many works \cite{chen2019fast,shi2019pointrcnn} apply an R-CNN-style two-stage detection paradigm. Point R-CNN \cite{shi2019pointrcnn} propose 3D RoIAlign to aggregate regional features based on the proposals and then refines the detections. PV-RCNN \cite{shi2020pv} and Voxel R-CNN \cite{deng2021voxel} construct two-parallel branches to extract both point-level and voxel-level features to enjoy the best of each. However, independently localizing moving instances can introduce misalignment noise, 3D-MAN \cite{yang20213d} and MPPNet \cite{chen2022mppnet} leverage multi-frame information to further enhance predictions with temporal knowledge. 
% Considering various architectures of LiDAR-based detectors, it may be hard to design a unified approach for SSOD, unless projects all information into a shared space, i.e., pseudo-labels.

\begin{figure*}[!t]
\begin{center}
\includegraphics[width=\textwidth]{images/framework.png}
\end{center}
\caption{The overall architecture of the proposed NoiseDet. It consists of two main components: noise-resistant instance supervision and dense feature consistency constraint. It follows the pseudo-labeling practice with a two-stage training paradigm: (i) pseudo labels are pre-generated with a well-trained teacher model on the unlabeled dataset, and (ii) the student model is trained on both labeled (omitted in the figure) and unlabeled LiDAR points in a semi-supervised manner.}
\label{fig:framework}
\end{figure*}

\subsection{Semi-Supervised Learning (SSL)}

Semi-supervised learning is an important task in leveraging easy-to-access unlabeled data to improve the supervised model. Most current SSL methods \cite{zhang2021flexmatch,grandvalet2004semi,chen2020big,han2018co} involve adding additional supervision on unlabeled data to regularize the learning of the model. Among them, pseudo-labeling is a popular pipeline \cite{cascante2021curriculum,lee2013pseudo,guo2018curriculumnet}, where unlabeled data is firstly labeled with a supervised model, and then acts in a common training paradigm. In order to guarantee the quality of the generated labels, \cite{lee2013pseudo} often filter them with a hard threshold based on the classification score. In addition to hard pseudo-labels, NoisyStudent \cite{xie2020self} explores soft supervision to avoid ambiguity problems. Besides, it injects different augmentations to the student and teacher models, to encourage consistency regularization. In light of this, plenty of approaches \cite{xie2020unsupervised,berthelot2019mixmatch,li2020dividemix} enforce the model to predict similar results when applying various input permutations. Such strategies are also verified on 2D object detection, where \cite{liu2021unbiased} borrows the idea from FixMatch to achieve promising performance. MUM \cite{kim2022mum} introduces Mix/UnMix augmentation, enforcing students to reconstruct unmixed features for the mixed input images. 

\subsection{Semi-Supervised 3D Object Detection}

Semi-supervised learning (SSL) has been rapidly developed in both classification and object detection domains and obtains promising results in recent years. There are two main streams in SSOD: consistency learning and pseudo labeling. Consistency-based works \cite{tarvainen2017mean,li2022pseco} apply data augmentations/perturbations to the input, which forms natural regularization for the network predictions. Such a consistency-learning target enforces the model to acquire valid information from the unlabeled data, therefore improving the performance. SESS \cite{zhao2020sess} is the first work to attempt such a paradigm on 3D object detection, where the classification and regression predictions are matched through L2 distance and supervised with the similarity loss on the teacher and student. Inspired by Mean Teacher \cite{tarvainen2017mean}, it also adopts the exponential moving average (EMA) technique to further boost the performance. Apart from the consistency-based approaches, pseudo-labeling is another solution \cite{xu2021semi,wang20213dioumatch}. Most PL works pay attention to the quality enhancement of pseudo labels. 3DIoUMatch \cite{wang20213dioumatch} proposes to learn the IoU of the network predictions and utilize it to adaptively filter the low-quality pseudo labels. In order to remove the duplicate score threshold search, ProficientTeacher \cite{yin2022semi} introduces a novel clustering-based box voting module, replacing the hand-crafted NMS process. Different from the previous approaches, our method views pseudo-labeling as a noisy learning problem, therefore delivering more generalization against noisy pseudo-data.


